Learning-based Efficient Graph Similarity Computation via Multi-Scale Convolutional Set Matching

Graph similarity computation is one of the core operations in many graph-based applications, such as graph similarity search, graph database analysis, graph clustering, etc. Since computing the exact distance/similarity between two graphs is typically NP-hard, a series of approximate methods have been proposed with a trade-off between accuracy and speed. Recently, several data-driven approaches based on neural networks have been proposed, most of which model the graph-graph similarity as the inner product of their graph-level representations, with different techniques proposed for generating one embedding per graph. However, using one fixed-dimensional embedding per graph may fail to fully capture graphs in varying sizes and link structures, a limitation that is especially problematic for the task of graph similarity computation, where the goal is to find the fine-grained difference between two graphs. In this paper, we address the problem of graph similarity computation from another perspective, by directly matching two sets of node embeddings without the need to use fixed-dimensional vectors to represent whole graphs for their similarity computation. The model, GraphSim, achieves the state-of-the-art performance on four real-world graph datasets under six out of eight settings (here we count a specific dataset and metric combination as one setting), compared to existing popular methods for approximate Graph Edit Distance (GED) and Maximum Common Subgraph (MCS) computation.

==> sec-vis.tex <==
\section{Visualizations}

To see how well \model ranks the graphs in the training set for query graphs in the test set, we show four example queries in Fig.~\ref{fig:search_demo}. In each demo, the top row depicts the query along with the ground-truth ranking results, labeled with their normalized GEDs to the query. The bottom row shows the graphs returned by our model, each with its rank shown at the top. 
% \model is able to retrieve graphs similar to the query. For example, in the case of Linux (Fig.~\ref{fig:search_demo_Linux}), the top 6 results are exactly the isomorphic graphs to the query.

A few more visualizations are included in Fig.~\ref{fig:search_demo_extra_1}, \ref{fig:search_demo_extra_2}, \ref{fig:search_demo_extra_3}, \ref{fig:search_demo_extra_4}, and \ref{fig:search_demo_extra_5}. In each figure, two similarity matrices are visualized, the left showing the similarity matrix between the query graph and the most similar graph, the right showing the similarity matrix between the query and the least similar graph. 

\begin{figure}[h]
    \centering
    \subfloat[Query ranking result.]
    {{\includegraphics[scale=0.57]{demo_1}}}
    \vspace{-0.0in}
    \centering
    \subfloat[Similarity matrix between the query and the most similar graph ranked by both methods.]
    {{\includegraphics[scale=0.4]{mne_1_1}}}
    \vspace{-0.0in}
    \centering
    \subfloat[Similarity matrix between the query and the least similar graph ranked by both methods.]
    {{\includegraphics[scale=0.4]{mne_1_2}}}
    \vspace{-0.0in}
    \caption{A query case study on AIDS.}
    \label{fig:search_demo_extra_1}
\end{figure}

\begin{figure}[h]
    \centering
    \subfloat[Query ranking result.]
    {{\includegraphics[scale=0.57]{demo_2}}}
    \vspace{-0.0in}
    \centering
    \subfloat[Similarity matrix between the query and the most similar graph ranked by both methods.]
    {{\includegraphics[scale=0.4]{mne_2_1}}}
    \vspace{-0.0in}
    \centering
    \subfloat[Similarity matrix between the query and the least similar graph ranked by both methods.]
    {{\includegraphics[scale=0.4]{mne_2_2}}}
    \vspace{-0.0in}
    \caption{A query case study on AIDS.}
    \label{fig:search_demo_extra_2}
\end{figure}

\begin{figure}[h]
    \centering
    \subfloat[Query ranking result.]
    {{\includegraphics[scale=0.57]{demo_3}}}
    \vspace{-0.0in}
    \centering
    \subfloat[Similarity matrix between the query and the most similar graph ranked by both methods.]
    {{\includegraphics[scale=0.4]{mne_3_1}}}
    \vspace{-0.0in}
    \centering
    \subfloat[Similarity matrix between the query and the least similar graph ranked by both methods.]
    {{\includegraphics[scale=0.4]{mne_3_2}}}
    \vspace{-0.0in}
    \caption{A query case study on AIDS.}
    \label{fig:search_demo_extra_3}
\end{figure}

\begin{figure}[h]
    \centering
    \subfloat[Query ranking result.]
    {{\includegraphics[scale=0.57]{demo_4}}}
    \vspace{-0.0in}
    \centering
    \subfloat[Similarity matrix between the query and the most similar graph ranked by both methods.]
    {{\includegraphics[scale=0.4]{mne_4_1}}}
    \vspace{-0.0in}
    \centering
    \subfloat[Similarity matrix between the query and the least similar graph ranked by both methods.]
    {{\includegraphics[scale=0.4]{mne_4_2}}}
    \vspace{-0.0in}
    \caption{A query case study on LINUX.}
    \label{fig:search_demo_extra_4}
\end{figure}

\begin{figure}[h]
    \centering
    \subfloat[Query ranking result.]
    {{\includegraphics[scale=0.57]{demo_5}}}
    \vspace{-0.0in}
    \centering
    \subfloat[Similarity matrix between the query and the most similar graph ranked by both methods.]
    {{\includegraphics[scale=0.4]{mne_5_1}}}
    \vspace{-0.0in}
    \centering
    \subfloat[Similarity matrix between the query and the least similar graph ranked by both methods.]
    {{\includegraphics[scale=0.4]{mne_5_2}}}
    \vspace{-0.0in}
    \caption{A query case study on LINUX.}
    \label{fig:search_demo_extra_5}
\end{figure}
